Optimal Sets and Solution Paths of ReLU Networks

We develop an analytical framework to characterize the set of optimal ReLU neural networks by reformulating the non-convex training problem as a convex program. We show that the global optima of the convex parameterization are given by a polyhedral set and then extend this characterization to the optimal set of the non-convex training objective. Since all stationary points of the ReLU training problem can be represented as optima of sub-sampled convex programs, our work provides a general expression for all critical points of the non-convex objective. We then leverage our results to provide an optimal pruning algorithm for computing minimal networks, establish conditions for the regularization path of ReLU networks to be continuous, and develop sensitivity results for minimal ReLU networks.

==> appendices/conjectures.tex <==
%!TEX root=../main.tex
\begin{proposition}\label{prop:proximal-gradient}
	The proximal-gradient algorithm with update rule
	\begin{equation}\label{eq:proximal-gradient}
		\begin{aligned}
			\wplus   & = \wk - \eta \nabla f(\w^k)                                          \\
			\w^{k+1} & =  \frac{\wplus}{\norm{\wplus}_2}(\norm{\wplus}_2 - \eta \lambda)_+,
		\end{aligned}
	\end{equation}
	and initialized at \( \w^0 \in \Row(X) \) converges to the min-norm solution \( \wmin(\lambda) \).
\end{proposition}
\begin{proof}
	The proof follows by showing that \( \w^{k} \in \Row(X) \)
	for all \( k \geq 0 \), which implies \( \w^{k}_\acts \in \Row(\Xas) \).
	As a result, the limit --- which is known to be a solution by standard
	optimization theory --- satisfies \( \lim_k \w^k \in \Row(\Xas) \).
	This condition uniquely identifies the min-norm solution,
	which yields the desired result.

	Assume that \( \w^k \in \Row(X) \) and observe that
	\[
		\wplus = \wk - \eta X^\top (X w - y),
	\]
	implies \( \wplus \in \Row(X) \) as well.
	Given \( \wplus \), \( \w^{k+1} \) is the unique solution to the following
	optimization problem
	\[
		\w^{k+1} =
		\argmin_{w} \cbr{
			\lambda \sum_{\bi \in \calB} \norm{\wi}_2 +
			\frac{1}{2\eta}\norm{\w - \wplus}_2^2.
		}
	\]
	Optimality conditions imply \( \w^{k+1} + \eta \lambda v = \wplus \),
	where \( \vi \in \lambda \partial \norm{\wi^{k+1}}_2 \).
	This immediately implies \( w^{k+1} + \eta \lambda v \in \Row(X) \).
	Now, suppose \( \w^{k+1} = a + b \), where \( a \in \Row(X) \) and
	\( b \in \Null(X) \).
	Clearly if \( \wi = 0 \), then \( b_\bi = 0 \) must also hold.
	If \( \wi \neq 0 \), then
	by definition of \( \partial \norm{\wi}_2 \), we have
	\[
		a_\bi + b_\bi + \eta \lambda \frac{a_\bi + b_\bi}{\norm{a_\bi + b_\bi}_2}
		= \wplus_\bi.
	\]
	The issue now is that \( a_\bi \) and \( b_\bi \) are not necessarily
	orthogonal; \( a_\bi \in \Row(\Xbi) \), but \( b_\bi \) is not necessarily in
	\( \Null(\Xbi) \).
	I am currently stuck here.
\end{proof}

\begin{lemma}
	Let \( \lambda > 0 \).
	and suppose the equicorrelation set is \( \equi \).
	Then the solution to the  dual problem
	is the same as the solution to
	\begin{equation}\label{eq:reduced-dual}
		\begin{aligned}
			\max_{\eta} \;
			 & - \half (\eta - X^\top y) (X^\top X)^+ (\eta - X^\top y) + \half \norm{y}_2^2                               \\
			 & \quad \quad \text{s.t.} \quad \eta \in \Row(X), \; \norm{\eta_\bi}_2 = \lambda \; \forall \; \bi \in \equi.
		\end{aligned}
	\end{equation}
\end{lemma}
\begin{proof}
	Let \( \eta^* \) be a solution to the dual problem
	and \( \eta' \) a solution to the dual problem with reduced constraints.
	Let \( d^* \) be the optimal value of the dual problem and \( d' \) the
	optimal value of the reduced problem.
	Observe that \( d' \geq d^* \) since \( \eta^* \) is feasible for the
	reduced problem.

	Assume that \( \eta'_\bi \geq \lambda \) for some \( \bi \in \calB \setminus \calE \).
	Since \( \eta^*_\bi < \lambda \), there exists \( \alpha > 0 \)
	such that
	\[
		\bar \eta = \alpha \eta^* + (1- \alpha) \eta',
	\]
	is feasible.
	Moreover, the objective obtained by \( \bar \eta \) satisfies
	\[
		- \half (\bar \eta - X^\top y) (X^\top X)^+ (\bar \eta - X^\top y) + \half \norm{y}_2^2                              \geq \alpha d' + (1 - \alpha) d^*,
	\]
	by concavity, which implies that \( \bar \eta \) is a solution to the dual problem.
	However, the dual solution to the dual problem is exactly the block correlation
	vector, which is unique.
	This is a contradiction, so we conclude that \( \eta' \) is feasible
	for the dual problem.
	Feasibility combined with \( d' \geq d^* \) implies \( d' = d^* \)
	and \( \eta' = \eta^* \).
\end{proof}

The KKT conditions for constraint reduced dual problem are
\begin{equation}\label{eq:dual-kkt-conditions}
	\begin{aligned}
		(X^\top X)^+ (\eta - X^\top y)
		+ (I - X X^+) \beta
		+ \sum_{\bi \in \equi} \alpha_\bi \frac{\wi}{\norm{\eta_\bi}_2}
		                               & = 0                                       \\
		(I - X X^+) \eta + X X^+ \beta & = 0                                       \\
		\norm{\wi}_2                   & = \lambda \quad \forall \; \bi \in \equi.
	\end{aligned}
\end{equation}

The Jacobian of this system is
\begin{equation}
	J =
	\begin{bmatrix}
		(X^\top X)^+ & (I - X X^+) & D(\eta) \eta \\
		(I - X X^+)  & X X^+       & 0            \\
		D(\eta) \eta & 0           & 0
	\end{bmatrix},
\end{equation}
where \( D(\eta) \) is a block-diagonal matrix with blocks given by
\( D_\bi(w) = I / \norm{\wi}_2 \) if \( \eta \in \equi \)
and \( D_\bi(w) = 0 \) otherwise.

\begin{proposition}
	The Jacobian of the constraint reduced problem is invertible
	for every \( \bar \eta, \bar \beta, \bar \alpha \).
\end{proposition}
\begin{proof}
	Suppose there exists \( \eta, \beta, \alpha \) such that
	\[
		\begin{bmatrix}
			(X^\top X)^+           & (I - X X^+) & D(\bar \eta) \bar \eta \\
			(I - X X^+)            & X X^+       & 0                      \\
			D(\bar \eta) \bar \eta & 0           & 0
		\end{bmatrix}
		\begin{bmatrix}
			\eta  \\
			\beta \\
			\alpha
		\end{bmatrix}
		= 0.
	\]
	For \( \we \)
\end{proof}

%\solutionFunction*
%\begin{proof}
%    For ease of notation, let
%    \[
%        \calX =
%        \cbr{
%            w \in \R^d : \we = \wmin_\equi(\lambda) + z,
%            z \in \calN_\lambda, \,
%            w_{\inact} = 0, \,
%            \wi \neq 0 \implies \frac{\lambda \wi}{\norm{\wi}_2} = \ci(\lambda)
%        }.
%    \]
%    Recall that \( \hat y = X w \) is constant over \( \solfn(\lambda) \) and each
%    \( w \in \solfn(\lambda) \) can only have support on \( \equi \) by FO conditions.
%    Dropping the zero entries of \( w \), \( \hat y = \Xe \we \) and we deduce that
%    \[
%        z = \we - \wmin_\equi \in \Null(\Xe),
%    \]
%    for every \( w \in \solfn(\lambda) \).
%    Let us show that \( z \in \calN_\lambda \).

%    If \( \wmin_\bi \neq 0 \), then first order optimality conditions require
%    \[
%        \frac{\wmin_\bi}{\norm{\wmin_\bi}_2} = \lambda \cdot \ci,
%    \]
%    from which we have \( \wmin_\bi \in \Span(\ci) \).
%    Thus, \( \wi = 0 \) implies \( z_\bi = -\wmin_\bi \in \Span(\ci) \)
%    (this also trivially holds when \( \wmin_\bi = 0 \)).

%    Otherwise, if \( \wi \neq 0 \),
%    then first-order optimality again implies
%    \begin{align*}
%        \frac{\wi}{\norm{\wi}_2}   & = \lambda \cdot \ci \\
%        \implies \wmin_\bi + z_\bi & \in \Span(\ci)      \\
%        \implies z_\bi             & \in \Span(\ci),
%    \end{align*}
%    since \( \wmin_\bi \in \Span(\ci) \).
%    As a result, \( z \in \calN_\lambda \).
%    It is straightforward to check that first-order optimality implies
%    \( w_\inact = 0 \) so that \( \calW^* \subseteq \calX \).

%    For the reverse inclusion, let \( w \in \calX \).
%    Clearly
%    \[
%        X w = \Xe \we = \Xe \wmin_\equi = \hat y(\lambda),
%    \]
%    so that \( w \) has the correct model fit.
%    If \( \wi = 0 \) and \( i \in \inact \), then
%    \[
%        \norm{\Xbi^\top (y - X w)}_2 = \norm{\ci}_2 \leq \lambda,
%    \]
%    showing FO conditions are satisfied.
%    Alternatively, if \( i \in \equi \), then \( \Xbi^\top (y - X w) = \ci \)
%    and FO conditions are satisfied again.
%    Finally, we check blocks for which \( \wi \neq 0 \).
%    Membership in \( \calX \) implies
%    \[
%        \frac{\wi}{\norm{\wi}_2} = \ci
%    \]
%    and \( \wi \) again satisfies first-order optimality conditions.
%    Putting these conditions together implies \( w \in \solfn \).
%    This completes the proof.
%\end{proof}

\begin{restatable}{proposition}{maxSupport}\label{prop:max-support}
	\textcolor{red}{WARNING: This result is out of date and cannot be relied on.}\\

	The min-norm solution is supported on \( \equi \) for almost
	every \( y \).
	As a result, \( \wmin \) has largest support (i.e most non-zero blocks) of
	any solution for almost every \( y \).
\end{restatable}
\begin{proof}
	By \cref{lemma:min-norm-expression},
	\[
		\wmin_{\equi} = (\Xe^\top \Xe)^+\sbr{\Xe^\top y - \ve(\lambda)},
	\]
	where \( \vi \in \lambda \partial \norm{\wi^*}_2 \) is the subgradient
	of the min-norm solution.
	As a result, we observe that a block in the equicorrelation set is zero
	if and only if
	\begin{equation}\label{eq:zero-entry}
		(\Xe^\top \Xe)^+_\bi \Xe^\top y  = (\Xe^\top \Xe)^+_\bi \ve(\lambda).
	\end{equation}
	Note that \( \norm{\vi}_2 = \lambda \) since \( \bi \in \equi \),
	meaning \( \norm{\ve}_2 = \lambda \sqrt{\abs{\equi}} \).
	As a result,
	\[
		\calS = \cbr{ (\Xe^\top \Xe)^+_\bi z :
			\norm{z}_2 = \lambda \sqrt{\abs{\equi}}
		},
	\]
	defines the shell of an ellipsoid which is strictly larger than the set of \( \ve(\lambda) \) vectors as \( y \) ranges over \( \R^n \).
	The inverse image of this shell under \( (\Xe^\top \Xe)^+_\bi \) is
	\[
		[(\Xe^\top \Xe)^+_\bi]^{-1} \calS
		= \cbr{z + x
			: \norm{z}_2 = \lambda \sqrt{\abs{\equi}},
			x \in \Null((\Xe^\top \Xe)^+_\bi)}
	\]
	The condition in \cref{eq:zero-entry} is equivalent to
	\[
		\Xe^\top y \in [(\Xe^\top \Xe)^+_\bi]^{-1} \calS.
	\]
	Splitting \( \Xe^\top y = c + d \), \( c \in \Row((\Xe^\top \Xe)^+_\bi) \)
	and \( d \in \Null((\Xe^\top \Xe)^+_\bi) \),
	the inclusion is satisfied when \( \norm{c}_2 = \lambda \sqrt{\abs{\equi}} \).
	This event is measure zero under any continuous probability distribution,
	which proves \( \wmin_\bi \neq 0 \) for almost every \( y \).

	We have shown that
	\( \wmin \) is supported on \( \equi \) for almost every \( y \).
	Since the largest support set any solution can have is \( \equi \),
	it holds that \( \wmin \) has the largest support of any solution
	for almost every \( y \).
\end{proof}


==> appendices/discontinuity.tex <==
%!TEX root=../main.tex

% \oneNeuron*
\begin{proof}
	\citet{mishkin2022convex} show that \autoref{eq:relu-least-squares} has the same global optimal values as
	\begin{equation*}
		\min_{v, \gamma \in \cbr{-1, 1}} \half \norm{\sum_{i=1}^p (X v_i)_+ \gamma - y} + \lambda \sum_{i = 1}^p \norm{w_i}_2,
	\end{equation*}
	with objective-preserving mapping \( w_i = v_i / \sqrt{\norm{v_i}_2} \),
	\( \alpha_i = \gamma_i \sqrt{\norm{v_i}_2} \).
	Thus, we shall analyze this equivalent problem when characterizing \( s(\lambda) \).

	Consider the case \( p = 1 \).
	Let \( X, y \) consist of two training points, \( (x_1, y_1) = (-100, 1) \) and \( (x_2, y_2) = (1, 10) \).
	In what follows, we drop the subscript for \( v \) and \( \gamma \) since \( p = 1 \) and we consider a one-dimensional.
	The optimization problem of interest is
	\begin{equation*}
		\min_{v, \gamma} \half \rbr{(x_1 v)_+ \gamma - y_1}^2 + \rbr{(x_2 v)_+ \gamma - y_2}^2 + \lambda \abs{v}.
	\end{equation*}
	Since \( x_1 < 0 \) and \( x_2 > 0 \), we can re-write this optimization problem as
	\[
		\min_{v, \gamma} \half \mathbbm{1}_{v \leq 0} \rbr{\rbr{x_1 v \gamma - y_1}^2 + y_2^2} + \mathbbm{1}_{v > 0}\rbr{\rbr{x_2 v \gamma - y_2}^2 + y_1^2} + \lambda \abs{v}.
	\]
	By inspection, we see that \( \gamma = +1 \) is optimal in both cases, leading to the following simplified expression:
	\[
		\min_{v} \half \mathbbm{1}_{v \leq 0} \rbr{\rbr{x_1 v - y_1}^2 + y_2^2} + \mathbbm{1}_{v > 0}\rbr{\rbr{x_2 v - y_2}^2 + y_1^2} + \lambda \abs{v}.
	\]
	This is a piece-wise continuous (but non-smooth) quadratic with a breakpoint at \( v^* = 0 \).
	We not determine the solution to this minimization problem via a case analysis.

	\textbf{Case 1}: \( v^* = 0 \).
	Then, the optimal objective is trivially \( f(v^*) = y_1^2 + y_2^2 \).

	\textbf{Case 2}: \( v^* < 0 \).
	First order optimality conditions are
	\[
		x_1 \rbr{x_1 v_{-}^* - y_1} - \lambda = 0 \implies v_{-1}^* = \frac{y_1 \cdot x_1 + \lambda}{x_1^2},
	\]
	which is valid only if \( \lambda < |y_1 \cdot x_1| = 100 \).
	The minimum objective value is then
	\begin{align*}
		\half \rbr{\rbr{x_1 v_{-}^* - y_1}^2 + y_2^2} - \lambda v_{-}^*
		 & = \rbr{\rbr{x_1 \frac{y_1 \cdot x_1 + \lambda}{x_1^2} - y_1}^2 + y_2^2} - \lambda \rbr{\frac{y_1 \cdot x_1 + \lambda}{x_1^2}} \\
		 & = \frac{\lambda^2}{x_1^2} + y_2^2 - \lambda \rbr{\frac{y_1 \cdot x_1 + \lambda}{x_1^2}}                                       \\
		 & = -\frac{\lambda y_1}{x_1} + y_2^2.
	\end{align*}

	\textbf{Case 3}: \( v_{+}^* > 0 \).
	Similarly to the previous case, we obtain
	\[
		x_2 \rbr{x_2 v_{+}^* - y_2} + \lambda = 0 \implies v_{+}^* = \frac{y_2 \cdot x_2 - \lambda}{x_2^2},
	\]
	which is valid only if \( \lambda < |y_2 \cdot x_2| = 10 \).
	In this case, the minimum objective is
	\begin{align*}
		\half \rbr{\rbr{x_2 v_{+}^* - y_2}^2 + y_1^2} + \lambda v_{+}^*
		 & = \rbr{\rbr{x_2 \frac{y_2 \cdot x_2 + \lambda}{x_2^2} - y_2}^2 + y_1^2} - \lambda \rbr{\frac{y_2 \cdot x_2 + \lambda}{x_2^2}} \\
		 & = \frac{\lambda^2}{x_2^2} + y_2^2 + \lambda \rbr{\frac{y_2 \cdot x_2 - \lambda}{x_2^2}}                                       \\
		 & = \frac{\lambda y_2}{x_2} + y_1^2.
	\end{align*}

	To combine the cases, observe that
	\begin{align*}
		f(v_+^*) - f(v_-^*)
		 & = \frac{\lambda y_2}{x_2} + y_1^2 - \sbr{-\frac{\lambda y_1}{x_1} + y_2^2} \\
		 & = \lambda \rbr{\frac{x_1 y_2 + x_2 y_1}{x_1 x_2}} + y_1^2 - y_2^2          \\
		 & = \lambda \rbr{\frac{-100 (10) + 1 (1)}{-100 (1)}} + 1 - 100               \\
		 & = 9.99 \lambda - 99.
	\end{align*}
	We deduce that \( f(v_+^*) - f(v_-^*) > 0 \) (and thus \( v^* \leq 0 \))
	whenever \( \lambda > 9.90990991 \approx 10 \).

	In particular, taking \( \lambda = 10 \), we find
	\[
		f(v_-^*) = 100 - 0.1 = 99.99 < 101 = y_1^2 + y_2^2 = f(0),
	\]
	so that \( v_-^* \) is optimal and \( s(10) = v_-^* < 0 \).
	Moreover, \( v_-^* \) is strictly decreasing as a function of \( \lambda \),
	for all \( \lambda > 9.90990991 \)
	so that \( v_-^* \)

	Now, consider \( \lambda = 9.90990991 - \epsilon \) to see that
	\[
		f(v_+^*) = 100.0990991 - 10 \epsilon < 101 = y_1^2 + y_2^2 = f(0),
	\]
	for all \( \epsilon > 0 \).
	We deduce that \( v_+^* > 0 \) is optimal for all \( \epsilon > 0 \) and
	thus \( s(\lambda) \) is discontinuous at \( \lambda = 9.90990991 \).
\end{proof}



==> appendices/group_lasso.tex <==
%!TEX root=../main.tex
\solutionFunctionAlt*
\begin{proof}
	Define
	\[
		\calX =
		\bigg\{ w \in \R^d :
		\wi = \alpha_\bi \ci, \alpha_\bi \geq 0, \forall \, \bi \in \equi, \,
		\wi = 0 \, \forall \, \bi \in \calB \setminus \equi,
		X w = \hat y.
		\bigg\}
	\]
	Let \( w \in \solfn(\lambda) \).
	If \( \wi \neq 0 \), then FO conditions imply
	\[
		\lambda \frac{\wi}{\norm{\wi}_2} = \ci \implies \wi = \alpha_\bi \ci,
	\]
	for \( \alpha > 0 \).
	If \( \wi = 0 \), then \( \wi = \alpha_\bi \ci \) holds trivially for
	\( \alpha_\bi = 0 \).
	Finally, since \( w \) is optimal, it must satisfy
	\[
		X \w = \hat y,
	\]
	which implies that \( w \in \calX \).

	Now, suppose that \( w' \in \calX \).
	Let's check FO conditions for \( w' \):
	if \( \wi \neq 0 \), then
	\begin{align*}
		\wi' = \alpha \ci
		 & \implies \frac{\wi'}{\norm{\wi'}_2} = \frac{\ci}{\lambda} \\
		 & \implies \lambda \frac{\wi'}{\norm{\wi'}_2} = \ci,
	\end{align*}
	where we have used the fact that \( \norm{\ci}_2 = \lambda \)
	for all \( \bi \in \equi \).
	If \( \wi' = 0 \), then
	\[
		X w' = \hat y \implies \norm{\Xbi^\top (y - Xw')}_2 \leq \lambda,
	\]
	which satisfies FO conditions.
	We conclude \( w' \in \solfn(\lambda) \).
\end{proof}


\begin{restatable}{lemma}{boundedSolutions}\label{lemma:bounded-solutions}
	The correlation vector \( v(\lambda) = X^\top (y -  X\wmin(\lambda)) \) is bounded
	for all \( \lambda \geq 0 \).
	Moreover, every solution to the group lasso problem
	is bounded by an absolute constant independent of \( \lambda \).
	Specifically, every \( w \in \solfn(\lambda) \) satisfies
	\[
		\sum_{\bi \in \calB} \norm{\wi}_2 \leq \sum_{\bi \in \calB} \norm{\bwi}_2.
	\]
	where \( \bar w \) is the min-norm least-squares solution.
\end{restatable}
\begin{proof}
	As noted, for \( \lambda = 0 \), the min-norm solution reduces to the min-norm least-squares
	solution and \( v(0) = 0 \) so that the claim trivial holds.
	For \( \lambda > 0 \), we show boundedness directly.
	Optimality of \( \wmin \) implies
	\[
		\half \norm{X \wmin - y}_2^2 + \lambda \sum_{\bi \in \calB} \norm{\wmin_\bi}_2
		\leq \half \norm{y}_2^2,
	\]
	from which we deduce the residual vector \( r(\lambda) \) is bounded
	for any choice of \( \lambda \).
	Thus, the block correlation vectors satisfy,
	\begin{align*}
		\norm{\vi(\lambda)}^2_2      & = \norm{\Xbi^\top r(\lambda)}_2^2                                   \\
		                             & \leq \norm{\Xbi}_2^2 \norm{y}_2^2                                   \\
		\implies \norm{v(\lambda)}_2 & \leq \sbr{\sum_{\bi \in \calB} \norm{\Xbi}^2_2 \norm{y}^2_2}^{1/2}.
	\end{align*}
	The right-hand quantity is independent of \( \lambda \) and
	so \( v(\lambda) \) is bounded for all \( \lambda \).

	Let \( h(w) = \sum_{\bi \in \calB} \norm{\wi}_2 \),
	and define \( W_{g} \) to be the set of least squares solutions with
	minimum group norm.
	That is,
	\[
		W_{g} = \argmin \cbr{h(w) : X^\top X w = X^\top y }.
	\]
	Let \( w_g \in W_g \),
	and suppose that \( h(w_{g}) < h(w(\lambda)) \)
	for some \( \lambda > 0 \), \( w \in \solfn(\lambda) \).
	Since
	\[
		\min_{w} \half \norm{X w - y}_2^2
		\leq \min_{w} \half \norm{X w - y}_2^2
		+ \lambda h(w),
	\]
	we deduce
	\[
		\half \norm{X w_g - y}_2^2 + \lambda h(w_g) <
		\half \norm{X \w(\lambda) - y}_2^2
		+ \lambda h(\w(\lambda)),
	\]
	which is a contradiction.
	So \( h(\w(\lambda)) \leq h(w_g) \) for all \( \lambda > 0 \).
	Observing \( h(w_g) \leq h(\bar w) \) by definition gives the result.
	Since \( h(\bar w) \) is independent of \( \lambda \),
	we conclude that \( \wmin(\lambda) \) is bounded.
\end{proof}


\subsection{Properties of the Solution Map}\label{app:solution-map}

\valueContinuity*
\begin{proof}
	Define the joint objective function
	\[
		f(w, \lambda) = \half \norm{X w - y}_2^2 + \lambda \sum_{b_i \in \calB} \norm{\wi}_2.
	\]
	Clearly \( f(w, \lambda) \) is jointly continuous in \( w \) and \( \lambda \).
	By \cref{lemma:bounded-solutions}, minimization of
	\( f(w, \lambda) \) over \( \R^d \) is equivalent to the
	constrained minimization problem,
	\[
		p^*(\lambda) = \min_{w} f(w, \lambda) \quad \text{s.t.} \; \sum_{\bi \in \calB} \norm{\wi}_2 \leq C,
	\]
	where \( C \) is a finite absolute constant.
	Note that this expression is also valid when \( \lambda = 0 \) as the
	min-norm solution to the unregularized least squares problem
	obeys the constraint.
	Thus, \( \solfn \) is a continuous optimization problem over a compact
	set and the classical result of \citet{berge1997topological}
	(see also \citet{hogan1973point}[Theorem 7]) implies
	\( p^* \) is continuous.
\end{proof}



\mapContinuity*
\begin{proof}
	The result follows from joint continuity of the objective
	\[
		f(w, \lambda) = \half \norm{X w - y}_2^2 + \lambda \sum_{b_i \in \calB} \norm{\wi}_2,
	\]
	and straightforward application of \citet{robinson1974sufficient}[Theorem 1].

	If \( X \) is full column rank, then the group lasso solution is
	unique for all \( \lambda \geq 0 \).
	The solution map is a singleton on \( \R^+ \) and closedness
	and openness are equivalent properties for singleton maps.
	Since we have already shown it is closed, the solution map
	must also be open.
	An identical argument shows that the solution map is open
	at every \( \lambda > 0 \) when GGP is satisfied.

	Now we show the reverse implication by proving the contrapositive.
	Assume \( X \) is not full column-rank.
	The solution map at \( \lambda = 0 \) is the solution set to the
	(unregularized) least squares problem,
	\[
		\min_w \half \norm{X w - y}_2^2,
	\]
	which is known to be \( \solfn(0) = \cbr{\wmin(0) + z : z \in \Null(X)} \).
	While \( \solfn(0) \) is unbounded, it holds that
	\( \solfn(\lambda) \subset C \) for some bounded \( C \) for
	every \( \lambda > 0 \) (\cref{lemma:bounded-solutions}).
	As a result, there exist uncountably many solutions in \( \solfn(0) \)
	which are not limit points of solutions in \( \solfn(\lambda_k) \)
	as \( \lambda_k \rightarrow 0 \).
	In other words, \( \solfn(0) \) is not open at \( 0 \).

	%Suppose \( X \) is not full column rank.
	%The solution map \( \solfn \) is open if and only if it is lower semi-continuous
	%\citep{hogan1973point}.
	%Recall that a point-to-set map \( T \) is lower semi-continuous at \( x \) if
	%for every open set \( S \), \( T(x) \cap S \neq \emptyset \), there
	%exists a neighborhood \( N(x) \) of \( x \) such that for all \( x' \in N(x) \),
	%\( T(x') \cap S \neq \emptyset \).

	%Suppose that \( \solfn \) is open from the right at \( \lambda = 0 \).
	%Standard results imply \( \text{aff}(\solfn(0)) = \Null(X) + w \),
	%where \( w \in \solfn(0) \).
	%We shall assume that \( w \) is dense.
	%By openness, for every \( \lambda_k \into 0 \), there exists
	%\( k' \),
	%and \( w(\lambda_k) \in \solfn(\lambda_k) \)
	%for \( k \geq k' \)
	%such that \( w(\lambda_k) \rightarrow w \).
	%Then \( w(\lambda_k) \) is also dense for sufficiently
	%large \( k \) and \( \calE_{\lambda_k} = \calB \).
	%\cref{cor:uniqueness-cond} now implies
	%\( \text{aff}(\solfn(\lambda')) \subset \Null(X) \) for all
	%\( \lambda' \) in a sufficiently small neighbourhood of
	%\( 0 \).

	%Since \( \solfn \) is open from the right at \( 0 \),
	%it is lower semi-continuous from the right.
	%Let
	%\[
	%    S = \text{relint}(\solfn(0))
	%    + B(0, \epsilon) \cap \Row(X),
	%\]
	%which is clearly open and satisfies
	%\( S \cap \solfn(0) = \text{relint}(\solfn(\lambda)) \),
	%which is always non-empty.
	%By lower semi-continuity, there exists a neighborhood
	%\( N(0) \) of \( 0 \) such that for every \( \lambda' \in N(0) \),
	%\( \solfn(\lambda') \cap S \neq 0 \).
	%That is, there exists \( w_1 \in \text{relint}(\solfn(0)), z_1 \in B(0, \epsilon) \cap \Row(X) \),
	%and \( w_2 \in \solfn(\lambda') \)
	%such that
	%\[
	%    w_1 + z_1 = w_2.
	%\]
	%But \( w_2 \) must be orthogonal to \( z_1 \)
	%since \( \text{aff}(w_2) \subset \Null(X) \).
	%Since \( w_1 \) is also orthogonal to \( z_1 \),
	%we conclude \( z_1 = 0 \) and \( w_1 = w_2 \).

	%However, this condition cannot happen because
	%\[
	%    \norm{\vi(0)}_2 = 0 \neq \lambda' = \norm{\vi(\lambda')}_2.
	%\]
	%So, the solution map is not open from the right at \( \lambda = 0 \).
\end{proof}




==> appendices/one_d.tex <==
%!TEX root=../main.tex


\begin{proposition}\label{prop:1d-to-lasso}
	Let \( Z \in \R^{n \times 1} \) be a one-dimensional training set
	and \( y \in \R^n \) the associated targets.
	The two-layer ReLU training problem with unregularized bias,
	\begin{equation}\label{eq:1d-relu}
		\begin{aligned}
			\min_{w_1, w_2, b} \half \norm{\sum_{i=1}^m (Z w_{1i} + b_{1i})_+ w_{2i} + b_2 - y}_2^2
			+ \frac{\lambda}{2} \norm{w_1}^2_2 + \norm{w_2}_2^2,
		\end{aligned}
	\end{equation}
	is equivalent to the following Lasso problem:
	\begin{equation}\label{eq:1d-bi-dual}
		\min_{v, b} \half \norm{A v + b - y} + \lambda \norm{v}_1,
	\end{equation}
	where
	\[
		A =
		\begin{bmatrix}
			0         & 0         & \ldots & 0             & Z_n - Z_1       & Z_{n-1} - Z_1     & \ldots & Z_2 - Z_1 \\
			Z_2 - Z_1 & 0         & \ldots & 0             & \vdots          & \vdots            & \ddots & 0         \\
			Z_3 - Z_1 & Z_3 - Z_2 & \ldots & 0             & \vdots          & \vdots            & \ddots & 0         \\
			\vdots    & \vdots    & \ddots & \vdots        & Z_{n} - Z_{n-2} & Z_{n-1} - Z_{n-2} & \ldots & 0         \\
			\vdots    & \vdots    & \ddots & 0             & Z_{n} - Z_{n-1} & 0                 & \ldots & 0         \\
			Z_n - Z_1 & Z_n - Z_2 & \ldots & Z_n - Z_{n-1} & 0               & 0                 & \ldots & 0
		\end{bmatrix}
	\]
	Finally, solutions to the Lasso problem can be mapped to solutions of the
	non-convex program as follows:
	\begin{equation}
		w_{1i}, w_{2i}, b_{1i} =
		\begin{cases}
			\frac{|v_i|}{\sqrt{|v_i|}}, \text{sign}(v_i) \sqrt{|v_i|}, - Z_i \frac{|v_i|}{\sqrt{|v_i|}} & \mbox{if \( v_i \neq 0, i \leq n-1 \)} \\
			-\frac{|v_i|}{\sqrt{|v_i|}}, \text{sign}(v_i) \sqrt{|v_i|}, Z_i \frac{|v_i|}{\sqrt{|v_i|}}  & \mbox{if \( v_i \neq 0, i \leq n-1 \)} \\
			0, 0, 0                                                                                     & \mbox{otherwise.}
		\end{cases}
	\end{equation}
	and \( b_2 = b \) represents the bias in the Lasso problem.

\end{proposition}
\begin{proof}
	Following \citet{pilanci2020convexnn},
	we observe that \cref{eq:1d-relu} is equivalent to the following constrained
	problem:
	\begin{equation}
		\begin{aligned}
			\min_{w_1, w_2, b_1, b_2} & \half \norm{\sum_{i=1}^m (Z w_{1i} + b_{1i})_+ w_{2i} + b_2 - y}_2^2 + \lambda \norm{w_2}_1 \\
			                          & \hspace{5em} \text{ s.t. } w_{1i} \in \cbr{+1 , -1}.
		\end{aligned}
	\end{equation}
	Now we introducing the constraint \( a = \sum_{i=1}^m (Z w_{1i} + b_{1i})_+ w_{2i} + b_2 \)
	so that we may compute the dual problem,
	\begin{align*}
		p^* & = \min_{w_1, w_2, b_1, b_2, a}
		\half \norm{a - y}_2^2 + \lambda \norm{w_1}^2_2 + \norm{w_2}_2^2                                                                                                    \\
		    & \hspace{5em} \text{ s.t. } a = \sum_{i=1}^m (Z w_{1i} + b_{1i})_+ w_{2i} + b_2, \, w_{1i} \in \cbr{+1, -1}
		\intertext{
			Forming the Lagrangian and infimizing over the primal parameters,
		}
		d(\eta)
		    & = \min_{w_1, w_2, b_1, b_2, a} \half \norm{a - y}_2^2 + \abr{\eta, a}
		+ \abr{\eta, \sum_{i=1}^m (Z w_{1i} + b_{1i})_+ w_{2i} + b_2} + \lambda \norm{w_2}_1 + \mathbbm{1}_{\cbr{+1, -1}^m}(w_{1})                                          \\
		    & = \min_{w_1, w_2, b_1, b_2} \half \norm{\eta - y}_2^2 + \half \norm{y}^2_2
		+ \abr{\eta, \sum_{i=1}^m (Z w_{1i} + b_{1i})_+ w_{2i} + b_2} + \lambda \norm{w_2}_1 + \mathbbm{1}_{\cbr{+1, -1}^m}(w_{1})                                          \\
		    & = \min_{w_1, w_2, b_1} \half \norm{\eta - y}_2^2 + \half \norm{y}^2_2
		+ \abr{\eta, \sum_{i=1}^m (Z w_{1i} + b_{1i})_+ w_{2i}} + \lambda \norm{w_2}_1 + \mathbbm{1}_{\cbr{+1, -1}^m}(w_{1}) - \mathbbm{1}_{\{0\}}(\eta^\top \mathbbm{1})   \\
		    & = \min_{w_1, w_2, b_1} \half \norm{\eta - y}_2^2 + \half \norm{y}^2_2
		+ \abr{w_{2}, (Z w_{1}^\top + b_{1i} \mathbbm{1})_+ \eta} + \lambda \norm{w_2}_1 + \mathbbm{1}_{\cbr{+1, -1}^m}(w_{1}) - \mathbbm{1}_{\{0\}}(\eta^\top \mathbbm{1}) \\
		    & = \min_{w_1, b_1} \half \norm{\eta - y}_2^2 + \half \norm{y}^2_2
		- \mathbbm{1}(\norm{(Z w_{1}^\top + b_{1i} \mathbbm{1})_+ \eta}_\infty \leq \lambda) + \mathbbm{1}_{\cbr{+1, -1}^m}(w_{1}) - \mathbbm{1}_{\{0\}}(\eta^\top \mathbbm{1}).
	\end{align*}
	Minimizing over \( w_1 \) and \( b_1 \) in the last equation is equivalent
	to including linear semi-infinite constraints in the optimization problem,
	\begin{equation}\label{eq:1d-dual}
		\begin{aligned}
			d(\eta)
			 & =  \half \norm{\eta - y}_2^2 + \half \norm{y}^2_2              \\
			 & \hspace{2em} \text{ s.t. } \sup_{w_{1i} \in \cbr{+1, -1}^m, b}
			\abs{\eta^\top (Z w_{1i} + b_{1i} \mathbbm{1})_+} \leq \lambda.
		\end{aligned}
	\end{equation}
	Note that the number of neurons \( m \) vanishes since it is sufficient
	for one neuron to attain the maximum and define the constraint set.

	Let us analyze the constraint set.
	First, observe that we may remove \( w_{1i} \) by splitting it its
	possible values as follows:
	\[
		\cbr{ \eta :
			\sup_{w_{1i} \in \cbr{+1, -1}^m, b}
			\abs{\eta^\top (Z w_{1i} - b \mathbbm{1})_+}
			\leq \lambda
		}
		=
		\cbr{ \eta :
			\sup_{b}
			\abs{\eta^\top (Z - b \mathbbm{1})_+}
			\leq \lambda, \,
			\sup_{b}
			\abs{\eta^\top (Z - b \mathbbm{1})_-},
		}
	\]
	Consider first the optimization problem
	\[
		\sup_{b}
		\abs{\eta^\top (Z - b \mathbbm{1})_+}
	\]
	This is maximization of a piece-wise linear objective
	over pieces \( [-\infty, Z_{(1)}],  \cbr{[Z_{(j)}, Z_{(j+1)}]}_{j = 1}^n, [Z_{(n)}, \infty] \).
	Since the optimization is an LP over each piece, the optimum must occur
	in the set \( \cbr{- \infty, \infty} \cup \cbr{Z_{(j)}}_{j=1}^n \).
	Clearly it does not occur at \( \infty \).
	Taking \( b \rightarrow -\infty \), we deduce the constraint
	\( \eta^\top \mathbbm{1} = 0 \), otherwise the dual is infeasible.
	Under this constraint, the optimum must occur at one of the breakpoints.
	Enumerating over all such values of \( b \) gives the following:
	\begin{align*}
		\sup_{b}
		\abs{\eta^\top (Z - b \mathbbm{1})_+}
		 & =
		\sup_{j}
		\abs{\eta^\top (Z + Z_{(j)} \mathbbm{1})_+}.
		\intertext{
			Assuming without loss of generalizing that \( Z \) is sorted
			in increasing order, we obtain
		}
		 & = \norm{\eta^\top A_1}_\infty,
	\end{align*}
	where
	\[
		A_1 =
		\begin{bmatrix}
			0         & 0         & \ldots & 0             \\
			Z_2 - Z_1 & 0         & \ldots & 0             \\
			Z_3 - Z_1 & Z_3 - Z_2 & \ldots & 0             \\
			\vdots    & \vdots    & \ddots & 0             \\
			Z_n - Z_1 & Z_n - Z_2 & \ldots & Z_n - Z_{n-1}
		\end{bmatrix}
	\]
	A similar analysis gives
	\[
		\sup_{b}
		\abs{\eta^\top (Z - b \mathbbm{1})_-}
		=
		\norm{\eta^\top A_2}_\infty,
	\]
	where \( A_2 \) is
	\[
		A_2 =
		\begin{bmatrix}
			Z_n - Z_1     & Z_{n-1} - Z_1     & \ldots & Z_2 - Z_1 \\
			\vdots        & \vdots            & \ldots & 0         \\
			Z_n - Z_{n-2} & Z_{n_1} - Z_{n-2} & \ldots & 0         \\
			Z_n - Z_{n-1} & 0                 & \ddots & 0         \\
			0             & 0                 & \ldots & 0
		\end{bmatrix}
	\]
	As a result, we may write the dual problem compactly as
	\begin{equation}\label{eq:1d-dual-compact}
		\begin{aligned}
			d(\eta)
			 & =  \half \norm{\eta - y}_2^2 + \half \norm{y}^2_2                                         \\
			 & \hspace{2em} \text{ s.t. } \abr{\eta, 1} = 0, \norm{\eta [A_1, A_2]}_\infty \leq \lambda.
		\end{aligned}
	\end{equation}
	We recognize \cref{eq:1d-dual-compact} as the dual of a Lasso problem with
	weight matrix \( \sbr{A_1; A_2} \).
	Indeed, it is straightforward to directly calculate that the bi-dual problem is
	\begin{equation}
		\min_{v} \half \norm{[A_1; A_2] v + b - y} + \lambda \norm{v}_2,
	\end{equation}
	where the \( \ell_1 \) penalty comes from the conjugate of the \( \ell_\infty \)-norm
	constraint and the bias stems from the \( \eta^\top \mathbbm{1} = 0 \)
	constraint.

	Now, observe that \( \eta = 0 \) strictly satisfies the constraint in \cref{eq:1d-dual-compact},
	Slater's constraint qualification holds, and strong duality attains.
	Thus, the bidual has the same optimal value as the dual program.
	\citet{pilanci2020convexnn} show that strong duality holds for the
	original non-convex training problem and its dual as long as \( m \geq m^* \).
	Thus, the bidual attains the same optimal value as
	\cref{eq:1d-relu} under this condition.

	It remains only to check the mapping between solutions of the bidual and the original
	non-convex program preserves objective values.
	This is straightforward to do by direct calculation.
\end{proof}

\begin{lemma}
	Consider the one-dimensional training problem in \cref{eq:1d-relu}
	and assume that all examples \( Z_i \) are distinct.
	Then the optimal neural network is p-unique when \( n = 2 \) or \( n = 3 \).
\end{lemma}
\begin{proof}
	First consider \( n = 2 \).
	In this case, the data matrix for the corresponding lasso problem is given
	by
	\[
		A =
		\begin{bmatrix}
			0         & Z_2 - Z_1 \\
			Z_2 - Z_1 & 0
		\end{bmatrix},
	\]
	which is square and full rank. Thus, the lasso problem admits a unique
	solution and the optimal neural network is p-unique.

	The proof is slightly more complicated for \( n = 3 \).
	The data matrix is
	\[
		A =
		\begin{bmatrix}
			0         & 0         & Z_3 - Z_1 & Z_2 - Z_1 \\
			Z_2 - Z_1 & 0         & Z_3 - Z_2 & 0         \\
			Z_3 - Z_1 & Z_3 - Z_2 & 0         & 0
		\end{bmatrix},
	\]
	We check for uniqueness by checking if the columns of \( A \) are in
	general position, which is known to be a sufficient condition for
	uniqueness \citep{tibshirani2013unique}.
	The columns of \( A \) are in general position if and only if
	there do not exist \( n+1 \) columns of \( A \)
	and signs \( s_i \in \cbr{+1, -1} \) such that
	\[
		s_j a_j \in \text{Aff} \rbr{\cbr{s_i a_i}_{i \in \calI \setminus j}},
	\]
	for any choice of \( j \in \calI \).
	It is straightforward to show this holds by direct calculation.

	Consider \( j = 4 \).
	Inclusion in the affine hull requires
	\[
		s_1 (Z_2 - Z_1) = \alpha_3 s_3 (Z_3 - Z_1),
	\]
	which implies \( s_1 = s_3 \) and \( \alpha_3 = \frac{Z_2 - Z_1}{Z_3 - Z_1} \).
	Similarly,
	\begin{align*}
		0
		 & = \alpha_1 s_1 (Z_2 - Z_1) + \alpha_3 s_3 (Z_3 - Z_2)                    \\
		 & = \alpha_1 s_1 (Z_2 - Z_1) + s_3 (Z_3 - Z_2) \frac{Z_2 - Z_1}{Z_3 - Z_1} \\
		 & = (\alpha_1 s_1 + s_3 \frac{Z_3 - Z_2}{Z_3 - Z_1}) (Z_2 - Z_1),
	\end{align*}
	which implies \( s_1 = - s_3 \) and \( \alpha_1 = \frac{Z_3 - Z_2}{Z_3 - Z_1} \).
	Now, observe that
	\[
		\alpha_1 + \alpha_3 = \frac{Z_3 - Z_2}{Z_3 - Z_1} + \frac{Z_2 - Z_1}{Z_3 - Z_1} = 1,
	\]
	so that \( \alpha_2 = 0 \) is required.
	Since \( Z_3 - Z_2 \neq Z_3 - Z_1 \) because the \( Z_i \) are distinct,
	we conclude that the affine inclusion does not hold.
	Arguing in this manner for each choice of column gives the result.
\end{proof}

\begin{conjecture}
	The solution is not p-unique for \( n \geq 4 \).
\end{conjecture}
\begin{proof}
	I'm not certain how to show this result.
	For general data values, it turns into a combinatorial problem over (i)
	which $n = 4$ vectors to select out of the five possible and (ii) what
	signs $s_i$ to choose.
\end{proof}

\begin{lemma}
    
\end{lemma}







==> macros/tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	/62f0144/
\\Di	math.tex	/^\\newcommand{\\Di}{\\calD_{\\bi}}$/;"	C
\\Dis	math.tex	/^\\newcommand{\\Dis}{\\Di^{*}}$/;"	C
\\Ds	math.tex	/^\\newcommand{\\Ds}{\\calD^{*}_\\lambda}$/;"	C
\\E	math.tex	/^\\newcommand{\\E}{\\bbE}$/;"	C
\\Ek	math.tex	/^\\newcommand{\\Ek}{\\bbE_{\\zk}}$/;"	C
\\Gs	math.tex	/^\\newcommand{\\Gs}{\\calG^{*}_{\\lambda}}$/;"	C
\\Ka	math.tex	/^\\newcommand{\\Ka}{K_\\act}$/;"	C
\\Kd	math.tex	/^\\newcommand{\\Kd}{K_{\\calD}}$/;"	C
\\Kda	math.tex	/^\\newcommand{\\Kda}{K_{\\calD \\cap \\act}}$/;"	C
\\Kdas	math.tex	/^\\newcommand{\\Kdas}{K_{\\Gs}}$/;"	C
\\Ki	math.tex	/^\\newcommand{\\Ki}{K_{\\bi}}$/;"	C
\\Kid	math.tex	/^\\newcommand{\\Kid}{K_{\\Di}}$/;"	C
\\Kids	math.tex	/^\\newcommand{\\Kids}{K_{\\Di^*}}$/;"	C
\\Lk	math.tex	/^\\newcommand{\\Lk}{L_{\\zk}}$/;"	C
\\Lmax	math.tex	/^\\newcommand{\\Lmax}{L_{\\text{max}}}$/;"	C
\\Lmin	math.tex	/^\\newcommand{\\Lmin}{L_{\\text{min}}}$/;"	C
\\Null	math.tex	/^\\newcommand{\\Null}{\\text{Null}}$/;"	C
\\R	math.tex	/^\\newcommand{\\R}{\\mathbb{R}}$/;"	C
\\Range	math.tex	/^\\newcommand{\\Range}{\\text{Range}}$/;"	C
\\Row	math.tex	/^\\newcommand{\\Row}{\\text{Row}}$/;"	C
\\Si	math.tex	/^\\newcommand{\\Si}{\\calN_{\\bi}}$/;"	C
\\Sis	math.tex	/^\\newcommand{\\Sis}{\\Ni^{*}}$/;"	C
\\Span	math.tex	/^\\newcommand{\\Span}{\\text{Span}}$/;"	C
\\Ss	math.tex	/^\\newcommand{\\Ss}{\\calN^{*}_\\lambda}$/;"	C
\\Var	math.tex	/^\\newcommand{\\Var}[1]{\\textbf{Var}\\sbr{#1}}$/;"	C
\\Xa	math.tex	/^\\newcommand{\\Xa}{X_\\act}$/;"	C
\\Xas	math.tex	/^\\newcommand{\\Xas}{X_\\acts}$/;"	C
\\Xbi	math.tex	/^\\newcommand{\\Xbi}{X_\\bi}$/;"	C
\\Xe	math.tex	/^\\newcommand{\\Xe}{X_\\equi}$/;"	C
\\Z	math.tex	/^\\newcommand{\\Z}{Z}$/;"	C
\\abr	math.tex	/^\\newcommand{\\abr}[1]{\\left\\langle#1\\right\\rangle}$/;"	C
\\abs	math.tex	/^\\newcommand{\\abs}[1]{\\left\\vert #1\\right\\vert}$/;"	C
\\act	math.tex	/^\\newcommand{\\act}{{\\calA_{\\lambda}}}$/;"	C
\\acts	math.tex	/^\\newcommand{\\acts}{{\\calA_{\\lambda}^{*}}}$/;"	C
\\addnumber	math.tex	/^\\newcommand{\\addnumber}{\\addtocounter{equation}{1}\\tag{\\theequation}}$/;"	C
\\alphak	math.tex	/^\\newcommand{\\alphak}{\\alpha_{k}}$/;"	C
\\alphakk	math.tex	/^\\newcommand{\\alphakk}{\\alpha_{k+1}}$/;"	C
\\argdot	math.tex	/^\\newcommand{\\argdot}{{\\,\\vcenter{\\hbox{\\tiny$\\bullet$}}\\,}} %generic argument dot$/;"	C
\\as	math.tex	/^\\newcommand{\\as}[1]{\\stackrel{\\text{\\rm\\tiny a.s.}}{#1}}$/;"	C
\\aside	paragraph.tex	/^\\newcommand{\\aside}[1]{(\\textcolor{red}{\\textbf{Aside}: #1})}$/;"	C
\\betak	math.tex	/^\\newcommand{\\betak}{\\beta_{k}}$/;"	C
\\betakk	math.tex	/^\\newcommand{\\betakk}{\\beta_{k+1}}$/;"	C
\\bi	math.tex	/^\\newcommand{\\bi}{{b_i}}$/;"	C
\\biggmid	math.tex	/^\\newcommand{\\biggmid}{\\bigg \\vert }$/;"	C
\\bwi	math.tex	/^\\newcommand{\\bwi}{\\bar{w}_\\bi}$/;"	C
\\ca	math.tex	/^\\newcommand{\\ca}{c_\\act}$/;"	C
\\cas	math.tex	/^\\newcommand{\\cas}{c_\\acts}$/;"	C
\\cbr	math.tex	/^\\newcommand{\\cbr}[1]{\\left\\{#1\\right\\}}$/;"	C
\\ce	math.tex	/^\\newcommand{\\ce}{c_\\equi}$/;"	C
\\ci	math.tex	/^\\newcommand{\\ci}{c_\\bi}$/;"	C
\\diag	math.tex	/^\\newcommand{\\diag}{\\text{diag}}$/;"	C
\\dist	math.tex	/^\\newcommand{\\dist}[1]{\\stackrel{\\text{\\rm\\tiny dist}}{#1}}$/;"	C
\\equas	math.tex	/^\\newcommand{\\equas}{\\stackrel{\\text{\\rm\\tiny a.s.}}{=}}$/;"	C
\\equdist	math.tex	/^\\newcommand{\\equdist}{\\stackrel{\\text{\\rm\\tiny dist}}{=}}$/;"	C
\\equi	math.tex	/^\\newcommand{\\equi}{{\\calE_{\\lambda}}}$/;"	C
\\etak	math.tex	/^\\newcommand{\\etak}{\\eta_k}$/;"	C
\\etakk	math.tex	/^\\newcommand{\\etakk}{\\eta_{k+1}}$/;"	C
\\etamax	math.tex	/^\\newcommand{\\etamax}{\\eta_{\\text{max}}}$/;"	C
\\etamin	math.tex	/^\\newcommand{\\etamin}{\\eta_{\\text{min}}}$/;"	C
\\f	math.tex	/^\\newcommand{\\f}{f}$/;"	C
\\fj	math.tex	/^\\newcommand{\\fj}{f_i}$/;"	C
\\fk	math.tex	/^\\newcommand{\\fk}{f_{i_k}}$/;"	C
\\fkk	math.tex	/^\\newcommand{\\fkk}{f_{i_{(k+1)}}}$/;"	C
\\fopt	math.tex	/^\\newcommand{\\fopt}{f^*}$/;"	C
\\grad	math.tex	/^\\newcommand{\\grad}{\\nabla f}$/;"	C
\\gradk	math.tex	/^\\newcommand{\\gradk}{\\nabla f_{i_k}}$/;"	C
\\gradkk	math.tex	/^\\newcommand{\\gradkk}{\\nabla f_{i_{(k+1)}}}$/;"	C
\\halved	math.tex	/^\\newcommand{\\halved}[1]{\\frac{#1}{2}}$/;"	C
\\inact	math.tex	/^\\newcommand{\\inact}{{\\calI_{\\lambda}}}$/;"	C
\\ind	math.tex	/^\\newcommand{\\ind}[0]{\\perp \\!\\!\\! \\perp }$/;"	C
\\into	math.tex	/^\\newcommand{\\into}{\\rightarrow}$/;"	C
\\inv	math.tex	/^\\newcommand{\\inv}[1]{\\frac{1}{#1}}$/;"	C
\\iter	math.tex	/^\\newcommand{\\iter}{k}$/;"	C
\\mumax	math.tex	/^\\newcommand{\\mumax}{\\mu_{\\text{max}}}$/;"	C
\\mumin	math.tex	/^\\newcommand{\\mumin}{\\mu_{\\text{min}}}$/;"	C
\\nnz	math.tex	/^\\newcommand{\\nnz}{\\text{nnz}}$/;"	C
\\oracle	math.tex	/^\\newcommand{\\oracle}{\\mbox{\\( \\calO \\)}}$/;"	C
\\ra	math.tex	/^\\newcommand{\\ra}{\\rho_{\\act}}$/;"	C
\\ract	math.tex	/^\\newcommand{\\ract}{\\rho_{\\act}}$/;"	C
\\racts	math.tex	/^\\newcommand{\\racts}{\\rho_{\\acts}}$/;"	C
\\rbr	math.tex	/^\\newcommand{\\rbr}[1]{\\left(#1\\right)}$/;"	C
\\rd	math.tex	/^\\newcommand{\\rd}{\\rho_{\\calD}}$/;"	C
\\rda	math.tex	/^\\newcommand{\\rda}{\\rho_{\\calD \\cap \\act}}$/;"	C
\\rdas	math.tex	/^\\newcommand{\\rdas}{\\rho_{\\Gs}}$/;"	C
\\ri	math.tex	/^\\newcommand{\\ri}{\\rho_{\\bi}}$/;"	C
\\rid	math.tex	/^\\newcommand{\\rid}{\\rho_{\\Di}}$/;"	C
\\rmin	math.tex	/^\\newcommand{\\rmin}{\\rho^*}$/;"	C
\\sbr	math.tex	/^\\newcommand{\\sbr}[1]{\\left[#1\\right]}$/;"	C
\\seq	math.tex	/^\\newcommand{\\seq}[1]{\\rbr{#1}}$/;"	C
\\sgc	math.tex	/^\\newcommand{\\sgc}{\\rho}$/;"	C
\\solfn	math.tex	/^\\newcommand{\\solfn}{\\calW^*}$/;"	C
\\tetak	math.tex	/^\\newcommand{\\tetak}{{\\tilde{\\eta}}_{k}}$/;"	C
\\tran	math.tex	/^\\newcommand{\\tran}{{\\calT_{\\lambda}}}$/;"	C
\\trans	math.tex	/^\\newcommand{\\trans}{{\\calT_{\\lambda}^{*}}}$/;"	C
\\va	math.tex	/^\\newcommand{\\va}{v_\\act}$/;"	C
\\vas	math.tex	/^\\newcommand{\\vas}{v_\\acts}$/;"	C
\\ve	math.tex	/^\\newcommand{\\ve}{v_\\equi}$/;"	C
\\vi	math.tex	/^\\newcommand{\\vi}{v_\\bi}$/;"	C
\\vk	math.tex	/^\\newcommand{\\vk}{v_k}$/;"	C
\\vkk	math.tex	/^\\newcommand{\\vkk}{v_{k+1}}$/;"	C
\\vmin	math.tex	/^\\newcommand{\\vmin}{v^*}$/;"	C
\\w	math.tex	/^\\newcommand{\\w}{w}$/;"	C
\\wa	math.tex	/^\\newcommand{\\wa}{w_\\act}$/;"	C
\\was	math.tex	/^\\newcommand{\\was}{w_\\acts}$/;"	C
\\wbar	math.tex	/^\\newcommand{\\wbar}{\\bar{w}}$/;"	C
\\we	math.tex	/^\\newcommand{\\we}{w_\\equi}$/;"	C
\\wgc	math.tex	/^\\newcommand{\\wgc}{\\alpha}$/;"	C
\\wi	math.tex	/^\\newcommand{\\wi}{w_\\bi}$/;"	C
\\wk	math.tex	/^\\newcommand{\\wk}{w_k}$/;"	C
\\wkk	math.tex	/^\\newcommand{\\wkk}{w_{k+1}}$/;"	C
\\wmin	math.tex	/^\\newcommand{\\wmin}{w^*}$/;"	C
\\wopt	math.tex	/^\\newcommand{\\wopt}{w^*}$/;"	C
\\wplus	math.tex	/^\\newcommand{\\wplus}{w^+}$/;"	C
\\x	math.tex	/^\\newcommand{\\x}{x}$/;"	C
\\xbar	math.tex	/^\\newcommand{\\xbar}{\\xbar{w}}$/;"	C
\\xk	math.tex	/^\\newcommand{\\xk}{x_k}$/;"	C
\\xkk	math.tex	/^\\newcommand{\\xkk}{x_{k+1}}$/;"	C
\\xopt	math.tex	/^\\newcommand{\\xopt}{x^*}$/;"	C
\\y	math.tex	/^\\newcommand{\\y}{y}$/;"	C
\\yk	math.tex	/^\\newcommand{\\yk}{y_k}$/;"	C
\\ykk	math.tex	/^\\newcommand{\\ykk}{y_{k+1}}$/;"	C
\\z	math.tex	/^\\newcommand{\\z}{z}$/;"	C
\\zi	math.tex	/^\\newcommand{\\zi}{z_\\bi}$/;"	C
\\zk	math.tex	/^\\newcommand{\\zk}{z_{k}}$/;"	C
\\zkk	math.tex	/^\\newcommand{\\zkk}{z_{k+1}}$/;"	C
macros	README.md	/^# macros$/;"	c


==> sections/discontinuity.tex <==
%!TEX root=../main.tex

We first consider the simple case where \( \calL(\hat y, y) = \half \norm{\hat y - y}_2^2 \) and \( R(w, \alpha) = \half \sum_{i = 1}^p \norm{w_i}_2^2 + \norm{\alpha_i}_2^2 \).
This is the standard setting with least-squares loss with weight-decay regularization.
With these choices, \cref{eq:non-convex-relu-mlp} becomes
\begin{equation}
	\label{eq:relu-least-squares}
	\min_{w, \alpha} \half \norm{\sum_{i=1}^p (X w_i)_+ \alpha_i - y} + \frac{\lambda}{2} \sum_{i = 1}^p \norm{w_i}_2^2 + \norm{\alpha_i}_2^2.
\end{equation}
Our first result demonstrates that the solution cannot be guaranteed to be continuous in this setting.
\begin{restatable}{proposition}{oneNeuron}\label{prop:one-neuron}
	There exists a training set \( (X, y) \) such that the solution function for \cref{eq:relu-least-squares} is discontinuous.
\end{restatable}


==> sections/group_lasso.tex <==
%!TEX root=../main.tex

\aaron{TODO: remove this section and incorporate text into ReLU section.}

Let \( X \in \R^{n \times d} \) be a data matrix, \( y \in \R^n \) the
associated vector of targets,
and \( \calB = \cbr{b_1, \ldots, b_m} \) a disjoint partition of the feature indices
\( \cbr{1, \ldots, d} \).
Given a regularization parameter \( \lambda \geq 0 \), the linear group lasso
solves the following regularized regression problem:
\begin{equation}\label{eq:group-lasso}
	p^*(\lambda) = \min_{w} \half \norm{X w - y}_2^2 + \lambda \sum_{b_i \in \calB} \norm{\wi}_2.
\end{equation}
Solutions to \cref{eq:group-lasso} are block sparse when \( \lambda \) is sufficiently large, meaning \( \wi = 0 \) for some subset of \( \bi \).
This is similar to the feature sparsity given by the lasso,
to which the group lasso naturally reduces when \( \bi = \cbr{i} \) for each
\( \bi \in \calB \).

Our primary interest in this work is the solution map or
``regularization path'',
\[
	\solfn(\lambda) := \argmin_w f_\lambda(w).
\]
For a general data matrix, \( f_\lambda \) is not strictly convex and
the linear group lasso problem may admit multiple solutions.
As such, \( \solfn \) is a point-to-set map and
only the min-norm solution,
\[
	\wmin(\lambda) = \argmin \cbr{ \norm{w}_2 : w \in \solfn(\lambda) },
\]
defines a function.
Even in the non-unique case, the model fit \( \hat y(\lambda) = X w \) is the
same for all \( w \in \solfn(\lambda) \) \citep[Lemma 2]{vaiter2012dof}.
Moreover, if \( \lambda > 0 \), then it is straightforward to deduce that the sum of group norms
\( \sum_{i \in \calB} \norm{\wi}_2 \) is also constant over \( \solfn(\lambda) \).
Uniqueness of \( \hat y(\lambda) \) extends to the residual vector
\( r(\lambda) = y - \hat y(\lambda) \)
and the block correlation vectors \( \ci(\lambda) = \Xbi^\top r(\lambda) \).
We write \( c \in \R^d \) as the concatenation of the \( \ci \)
blocks.

Unlike the lasso, the group lasso solution map is not piece-wise linear
in general \citep{yuan2006model}.
This prevents us from obtaining an explicit expression for the solution
path between transition point, where features enter or exit the active set.
We overcome this difficulty by relying only on an \emph{implicit} characterization
of the path provided by the implicit function theorem.
We start towards this goal by developing optimality conditions for the group
lasso problem.

Since \cref{eq:group-lasso} is a convex optimization problem, first-order (FO)
optimality conditions are both necessary and sufficient for weights \( w \)
to be globally optimal.
Sub-differentiating the optimization problem gives the following FO conditions:
\begin{equation}\label{eq:fo-optimality}
	\begin{aligned}
		\ci(\lambda) := \Xbi^\top (y - X w) \in
		\begin{cases}
			\cbr{\lambda \frac{\wi}{\norm{\wi}_2}} & \mbox{if \( \wi \neq 0 \)} \\
			\cbr{v : \norm{v}_2 \leq \lambda }     & \mbox{otherwise,}
		\end{cases}
	\end{aligned}
\end{equation}
showing that \( \wi = 0 \) when \( \norm{\ci}_2 < \lambda \).
As a result, the equicorrelation set
\begin{equation}\label{eq:equi}
	\equi := \cbr{\bi \in \calB : \norm{\Xbi^\top (y - Xw)}_2 = \lambda},
\end{equation}
contains all blocks which may be active for fixed \( \lambda \).
The complement of \( \equi \) in \( \calB \) is the inactive set,
denoted \( \inact \).
Our first result combines FO conditions with uniqueness of \( \hat y(\lambda) \)
to characterize the solution map in terms of \( \Null(\Xe) \).
\begin{restatable}{proposition}{solutionFunctionAlt}\label{prop:sol-fn-alt}
	Suppose \( \lambda > 0 \).
	Then the solution function for the group lasso is given by
	\begin{equation}
		\begin{aligned}
			\solfn(\lambda) =
			\bigg\{ w \in \R^d : \,
			 & \forall \, \bi \in \equi, \, \wi = \alpha_\bi \ci, \alpha_\bi \geq 0, \, \\
			 & \forall \, b_j \in \calB \setminus \equi, \w_{b_j} = 0, \,
			X w = \hat y.
			\bigg\}
		\end{aligned}
	\end{equation}
\end{restatable}
As an immediate consequence, the solution map is a particular subset
of directions in \( \Null(\Xe) \).
\begin{corollary}\label{cor:uniqueness-cond}
	If \( w, w' \in \solfn \),
	then \cref{prop:sol-fn-alt} implies
	\[
		w - w' \in \calN_\lambda := \Null(\Xe) \cap \cbr{z : \zi \in \Span(\ci), i \in \equi }.
	\]
	As a result, the group lasso solution is unique when \( \calN_\lambda = \emptyset \).
\end{corollary}
\cref{cor:uniqueness-cond} extends a similar result for the lasso
to the group lasso \citep[Eq. 9]{tibshirani2013unique} and
implies the group lasso solution is unique for all \( \lambda \geq 0 \) if
the columns of \( X \) are linearly independent;
however, we can also use it to obtain the following refined condition
for uniqueness.
%\begin{restatable}{proposition}{GGP}[Group General Position]\label{prop:unique-sol}
%    Suppose for every \( \calE \subseteq \calB \), \( \abs{\calE} \leq n +1 \),
%    there do not exist unit vectors \( \zi \in \R^{\abs{\bi}} \)
%    such that for any \( j \in \calE \),
%    \[
%        X_{b_j} z_{b_j} \in
%        \text{affine}(\cbr{\Xbi \zi : \bi \in \calE \setminus b_j}).
%    \]
%    Then the group lasso solution is unique for all \( \lambda > 0 \).
%\end{restatable}
We call this uniqueness condition \emph{group general position}
(GGP) because it naturally extends general position to groups of column vectors.
General position itself is an extension of affine independence and is sufficient for the lasso solution
to be unique \citep{tibshirani2013unique}.
We note that GGP is strictly weaker than linear independence of the columns of \( X \),
but neither implies nor is implied by general position (\cref{prop:general-position-relation}).

\subsection{Properties of the Solution Map}

Now we prove several general results about the solution map \( \solfn \).
First we provide standard definitions for continuity-type properties of
a point-to-set map.

\begin{definition}[Closed Map]
	A point-to-set map \( T : \calX \into \calZ \) is closed if
	\( \cbr{\xk} \subset \calX \), \( \xk \into \bar x \) and \( z_k \in T(\xk) \),
	\( z_k \into \bar z \) implies \( \bar z \in T(\bar x) \).
\end{definition}

\begin{definition}[Open Map]
	A point-to-set map \( T : \calX \into \calZ \) is open if
	\( \cbr{\xk} \subset \calX \), \( \xk \into \bar x \) and \( \bar z \in T(\bar x) \),
	implies there exists \( k' \in \bbN \), \( z_k \in T(\xk) \) for \( k \geq k' \),
	such that \( z_k \into \bar z \).
\end{definition}

We say that \( T \) is \emph{continuous} if it is both closed and open.
If \( T(x) \) is a singleton for all \( x \in \calX \),
then openness/closedness of \( T \) are equivalent to the standard
notion of continuity.

Our first result of this section establishes continuity of the optimal
objective value.

\begin{restatable}{proposition}{valueContinuity}\label{prop:value-continuity}
	The optimal function value \( p^* \) is continuous for all
	\( \lambda \geq 0 \).
\end{restatable}

By analyzing the dual problem, we can extend continuity to the
model fit and the sum of group norms.

%\begin{restatable}{proposition}{modelFitContinuity}\label{prop:model-fit-continuity}
%    The optimal model fit \( \hat y(\lambda)  \) is continuous for all \( \lambda \geq 0 \) the penalty \( \sum_{\bi \in \calB} \norm{\wi(\lambda)}_2 \) is continuous
%    for \( \lambda > 0 \).
%\end{restatable}

It is straightforward to extend this characterization to closedness
of \( \solfn \), but openness is not possible in the general setting.

\begin{restatable}{proposition}{mapContinuity}\label{prop:map-continuity}
	The solution map \( \solfn \) is closed on \( \R_+ \)
	and open on \( R^+ \) if only if \( X \) has full column rank.
	However, if GGP holds, then \( \solfn \) is open for every \( \lambda > 0 \).
\end{restatable}

Continuity of \( \solfn \) is impossible in the general setting because, as \citet{hogan1973point} shows, openness is essentially a stability property, one which cannot be satisfies when the equicorrelation set changes.
Continuity of the unique solution path is an immediate corollary of
these developments.

\begin{corollary}
	The group lasso solution is unique and continuous for every \( \lambda > 0 \)
	when GGP holds and is also continuous at \( \lambda = 0 \) when \( X \)
	is full column rank.
\end{corollary}


